Saturating the Data Processing Inequality for $\alpha-z$ Renyi Relative Entropy

It has been shown that the $\alpha-z$ R{\'e}nyi relative entropy satisfies the Data Processing Inequality (DPI) for a certain range of $\alpha$'s and $z$'s. Moreover, the range is completely characterized by Zhang in `20. We prove necessary and algebraically sufficient conditions to saturate the DPI for the $\alpha-z$ R{\'e}nyi relative entropy whenever $1<\alpha\leq 2$ and $\frac{\alpha}{2}\leq z\leq\alpha$. Moreover, these conditions coincide whenever $\alpha=z$.

==> notUsed.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%% Sufficiency of DPI (algebraically) %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Sufficient conditions on saturating DPI (algebraically)}\label{sufficient}
Conversely, if we assume that 
\begin{equation}
\sigma_A^{\frac{q}{2}}(\sigma_A^{\frac{q}{2}}\rho_A^p\sigma_A^{\frac{q}{2}})^{\left(\frac{1}{p+q}-1\right)}\sigma_A^{\frac{q}{2}} \otimes\mathbbm{1} = \sigma_{AB}^{\frac{q}{2}}(\sigma_{AB}^{\frac{q}{2}}\rho_{AB}^p\sigma_{AB}^{\frac{q}{2}})^{\left(\frac{1}{p+q}-1\right)}\sigma_{AB}^{\frac{q}{2}},
\end{equation}
then 
\begin{equation}
\rho_{AB}^p[\sigma_A^{\frac{q}{2}}(\sigma_A^{\frac{q}{2}}\rho_A^p\sigma_A^{\frac{q}{2}})^{\left(\frac{1}{p+q}-1\right)}\sigma_A^{\frac{q}{2}} \otimes\mathbbm{1}] = \rho_{AB}^p[\sigma_{AB}^{\frac{q}{2}}(\sigma_{AB}^{\frac{q}{2}}\rho_{AB}^p\sigma_{AB}^{\frac{q}{2}})^{\left(\frac{1}{p+q}-1\right)}\sigma_{AB}^{\frac{q}{2}}].
\end{equation}
Thus 
\begin{equation}
\mathrm{Tr}\left(\rho_{AB}^p[\sigma_A^{\frac{q}{2}}(\sigma_A^{\frac{q}{2}}\rho_A^p\sigma_A^{\frac{q}{2}})^v\sigma_A^{\frac{q}{2}} \otimes\mathbbm{1}]\right) = \mathrm{Tr}\left(\rho_{AB}^p[\sigma_{AB}^{\frac{q}{2}}(\sigma_{AB}^{\frac{q}{2}}\rho_{AB}^p\sigma_{AB}^{\frac{q}{2}})^{\left(\frac{1}{p+q}-1\right)}\sigma_{AB}^{\frac{q}{2}}]\right)
\end{equation}
implies that 
\begin{equation}
\mathrm{Tr}\left((\sigma_A^{\frac{q}{2}}\rho_A^p\sigma_A^{\frac{q}{2}})^{\left(\frac{1}{p+q}\right)} \right) = \mathrm{Tr}\left((\sigma_{AB}^{\frac{q}{2}}\rho_{AB}^p\sigma_{AB}^{\frac{q}{2}})^{\left(\frac{1}{p+q}\right)}\right). 
\end{equation}
Since $\log$ is an monotone function, we have that 
\begin{equation}
\log\left[\mathrm{Tr}\left((\sigma_A^{\frac{q}{2}}\rho_A^p\sigma_A^{\frac{q}{2}})^{\left(\frac{1}{p+q}\right)} \right)\right] = \log\left[\mathrm{Tr}\left((\sigma_{AB}^{\frac{q}{2}}\rho_{AB}^p\sigma_{AB}^{\frac{q}{2}})^{\left(\frac{1}{p+q}\right)}\right)\right], 
\end{equation}
and hence 
\begin{equation}
\frac{1}{\alpha-1}\log\left[\mathrm{Tr}\left((\sigma_A^{\frac{q}{2}}\rho_A^p\sigma_A^{\frac{q}{2}})^{\left(\frac{1}{p+q}\right)} \right)\right] = \frac{1}{\alpha-1}\log\left[\mathrm{Tr}\left((\sigma_{AB}^{\frac{q}{2}}\rho_{AB}^p\sigma_{AB}^{\frac{q}{2}})^{\left(\frac{1}{p+q}\right)}\right)\right]. 
\end{equation}
This directly means 
$$D_{\alpha,z}(\rho_{AB}||\sigma_{AB})=D_{\alpha,z}(\rho_{A}||\sigma_{A}), $$ 
whenever $p=\frac{\alpha}{z}$ and $q=\frac{1-\alpha}{z}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% Principle of Uniform Boundedness %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{theorem}[Principle of Uniform Boundedness]\label{PUB}
Supposed $\{T_\alpha\}$ is any family of bounded linear maps from a Banach space $V_1$ to a normed space $V_2$. Suppose that for each $\psi\in V_i$ there exists a constant $C_\psi$ such that $\|T_\alpha\psi\|\leq C_\psi$ for all $\alpha$. Then there exists a constant $C$ such that $\|T_\alpha\|\leq C$ for all $\alpha$. 
\end{theorem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% states and densities 1 to 1 correspondence %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{theorem}[\cite{QforMath} Proposition 19.8]\label{19.8}
Suppose $\rho$ is a density operator on $\cH$. Then the map $\Psi_\rho:\cB(\cH)\to\mathbbm{C}$ given by
$$\Psi_\rho(A)=\mathrm{Tr}(\rho A) $$ 
is a family of expectation values. 
\end{theorem}

\begin{proof}
We will show the 4 conditions from the definition of a family of expectation values mentioned in (\ref{family}). 
\begin{enumerate}
    \item $\Psi_\rho(\mathbbm{1})=\mathrm{Tr}(\rho\mathbbm{1})=\mathrm{Tr}(\rho)=1$. 
    \item For any self adjoint operator $A$, we have that $\Psi_\rho(A)=\mathrm{Tr}(\rho A)=\mathrm{Tr}(A\rho)=\mathrm{Tr}((\rho A)^*)=\overline{\mathrm{Tr}(\rho A)}$. Thus $\Psi_\rho(A)$ is real.
    \item Since $\rho$ is a density operator, we can consider the unique square root $\rho^{\frac{1}{2}}$ that is non-negative and also self adjoint. Since $\rho^{\frac{1}{2}}$ is trace class, i.e., $\mathrm{Tr}((\rho^{\frac{1}{2}})^*(\rho^{\frac{1}{2}}))<\infty$, and since the set of trace class operators form an ideal, it follows that for any self adjoint and non-negative operator $A$, we have that $A\rho^{\frac{1}{2}}$ is trace class to. Thus $\Psi_\rho(A)=\mathrm{Tr}(\rho A)=\mathrm{Tr}(\rho^{\frac{1}{2}}A\rho^{\frac{1}{2}})=\langle\rho^{\frac{1}{2}},A\rho^{\frac{1}{2}}\rangle_{HS}\geq0$, where $\langle\cdot,\cdot\rangle_{HS}$ is the Hilbert Schmidt inner product.
    \item Suppose $\|A_N\psi-A\psi\|\to 0$ for all $\psi\in\cH$. i.e., $A_n\psi$ converges in norm to $A\psi$, for all $\psi\in\cH$. This means for all $\epsilon_\psi>0$, there exists $N>0$ such that for all $n>N$, we have that $\|A_n\psi-A\psi\|<\epsilon_\psi$. Then
    \begin{align}
    \|A_n\psi\|&=\|A_n\psi-A\psi+A\psi\| \\
    &\leq \|A_n\psi-A\psi\|+\|A\psi\| \\
    &<C_\psi,    
    \end{align}
    for some constant $C_\psi$. Then $\|A_n\psi\|$ is bounded for each fixed $\psi$. So by the Principle of Uniform Boundedness Theorem, there exists a $C>0$ such that $\|A_n\|<C$. If we let $\{e_j\}$ be an orthonormal basis for $\cH$, we have that 
    \begin{align}
        |\langle e_j,\rho^{\frac{1}{2}}A_n\rho^{\frac{1}{2}}e_j\rangle| = &  |\langle \rho^{\frac{1}{2}}e_j,A_n\rho^{\frac{1}{2}}e_j\rangle| \\
        \leq & \|\rho^{\frac{1}{2}}e_j\|^2\|A_n\rho^{\frac{1}{2}}e_j\|^2 \\ \label{CS}
        \leq & \|A_n\|^2\|A_n\rho^{\frac{1}{2}}e_j\|^2 \\
        \leq & C^2 \|\rho^{\frac{1}{2}}e_j\|^2 \\
        \leq & C^2 \sum_j\|\rho^{\frac{1}{2}}e_j\|^2 \\
        = & C^2 \sum_j \langle \rho^{\frac{1}{2}}e_j,\rho^{\frac{1}{2}}e_j\rangle \\
        = & C^2 \sum_j \langle e_j,A_n\rho e_j\rangle \\
        = & C^2 \mathrm{Tr}(\rho) < \infty,
    \end{align} where (\ref{CS}) is by the Cauchy Schwartz inequality. 
    If we consider $\psi=\rho^{\frac{1}{2}}e_j\in\cH$, then we have that 
    \begin{align}
        \lim_{n\to\infty}\Psi_\rho(A_n) = & \lim_{n\to\infty} \mathrm{Tr}(\rho A_n) \\
        = & \lim_{n\to\infty}\mathrm{Tr}(\rho^{\frac{1}{2}}A_n\rho^{\frac{1}{2}}) \\
        = & \lim_{n\to\infty} \sum_{j}\langle \rho^{\frac{1}{2}}e_j,A_n\rho^{\frac{1}{2}}e_j\rangle \\
        = & \sum_{j}\lim_{n\to\infty} \langle \rho^{\frac{1}{2}}e_j,A_n\rho^{\frac{1}{2}}e_j\rangle \label{DCT} \\
        = & \sum_{j} \langle \rho^{\frac{1}{2}}e_j,\lim_{n\to\infty}A_n\rho^{\frac{1}{2}}e_j\rangle \\
        = & \sum_{j} \langle \rho^{\frac{1}{2}}e_j,A\rho^{\frac{1}{2}}e_j\rangle \\
        = & \mathrm{Tr}(\rho A) \\
        = & \Psi_\rho(A),
    \end{align}
    Where, (\ref{DCT}) is by the Dominating Convergence Theorem. Hence $\Psi_\rho(A_n)\to\Psi_\rho(A)$ as desired. 
\end{enumerate}
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% states and densities 1 to 1 correspondence %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


The proof of the following result:

\begin{theorem}[\cite{summaryPaper} Proposition 7]
Let $\alpha,z>0$ with $\alpha\neq1$. Set $p=\frac{\alpha}{z}$, $q=\frac{1-\alpha}{z}$, $s=\frac{1}{p+q}$, $K=I$, $A=\rho$, and $B=\sigma$. Then $D_{\alpha,z}$ is monotone under quantum channels on $\cP(\cH)$  (for any finite dimensional $\cH$) if and only if one of the following holds:
\begin{enumerate}
    \item $\alpha<1$ and $\Psi_{p,q,s}(A||B)$ is jointly concave.
    \item $\alpha>1$ and $\Psi_{p,q,s}(A||B)$ is jointly convex.
\end{enumerate}
\end{theorem}


\begin{proof}
Assume $\alpha>1$ and suppose $\Psi$ is jointly convex. By the Steinspring Dilation theorem, (\textcolor{red}{in thesis state the theorem earlier}) for each quantum channel $\Lambda$, there exists a Hilbert space $\cH_2$ such that $N_2$=dim($\cH_2)\leq(\text{dim}(\cH))^2$, a Unitary $U$ on $\cH\otimes\cH_2$, and a pure state $\delta\in\cH_2$ such that 
\begin{equation}
\Lambda(\gamma)=\mathrm{Tr}_2(U(\gamma\otimes\delta)U^*),
\end{equation}
where $\mathrm{Tr}_2$ denotes a partial trace over $\cH_2$. Let $dv$ denote the normalized Haar measure on $G(U)$, which denotes the group of all unitaries on $\cH_2$. Then 
\begin{equation}\label{intRep}
\Lambda(\gamma)\otimes\frac{\mathbbm{1}}{N_2}=\int_{G(U)}(1\otimes v)U(\gamma\otimes\delta)U^*(1\otimes v^*)dv.
\end{equation}
Since $\mathrm{Tr}(a\otimes b)=\mathrm{Tr}(a)\mathrm{Tr}(b)$, it follows that
\begin{equation}
\Psi(\Lambda(\rho)||\Lambda(\sigma))=\Psi\left(\Lambda(\rho)\otimes \frac{\mathbbm{1}}{N_2}||\Lambda(\sigma)\otimes\frac{\mathbbm{1}}{N_2}\right).
\end{equation}
By the joint convexity of $\Psi$ and by equation (\ref{intRep}), we have 
\begin{align}
    \Psi(\Lambda(\rho)||\Lambda(\sigma))=&\Psi\left(\Lambda(\rho)\otimes \frac{\mathbbm{1}}{N_2}||\Lambda(\sigma)\otimes\frac{\mathbbm{1}}{N_2}\right) \\
    \leq & \int_{G(U)}\Psi((1\otimes v)U(\rho\otimes\delta)U^*(1\otimes v^*), (1\otimes v)U(\sigma\otimes\delta)U^*(1\otimes v^*))dv \\
    = & \int_{G(U)}\Psi((\rho\otimes\delta), (\sigma\otimes\delta))dv \\
    = & \int \Psi(\rho,\sigma) dv \\
    = & \Psi(\rho,\sigma),
\end{align}
where we use the tensor property of the trace functional on the first equality, the joint convexity properties for the first inequality, the unitary invariance of the Haar measure and from the trace for the second equality, the tensor property on the third equality, and the normalization of the Haar measure for the last equality. This shows that $\Psi$ is monotone increasing under quantum channels, and hence by \ref{monotone}, the data processing inequality holds. 
Conversely, suppose the data processing inequality holds. For $\rho_1,\rho_2, \sigma_1,\sigma_2\in\cP(\cH)$ and for all $\lambda\in(0,1)$. Define $\Lambda:\cP(\cH\otimes\cH)\to\cP(\cH)$ by 
$\Lambda\begin{pmatrix}
    a & b \\
    c & d
\end{pmatrix}:=a + d$. Then $\Lambda$ is a quantum channel. (\textcolor{red}{prove it!}) So by assumption and by \ref{monotone}, we have that $\Psi(\rho||\sigma)\geq \Psi(\Lambda(\rho)||\Lambda(\sigma))$. This implies that 
$$\Psi(\rho||\lambda)\geq\Psi(\lambda\rho_1+(1-\lambda)\rho_2||\lambda\sigma_1+(1-\lambda)\sigma_2)=\lambda\Psi(\rho_1||\sigma_1)+(1-\lambda)\Psi(\rho_2||\sigma_2).$$
Hence joint convexity follows. For $\alpha<1$, we can prove joint concavity in a similar manner.  (\textcolor{red}{more details on the last equality here and include the details for the concavity part})
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  Convexity concavity argument from zhang paper
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{theorem}
\cite[Proposition 5]{CFLconjecture}
For any $K\in\cB(\cH)$, define a functional
\begin{equation}\label{reduced}
    \Upsilon_{p,s}(A):=\mathrm{Tr}(K^*A^pK)^s=\mathrm{Tr}|A^{\frac{p}{2}}K|^{2s}\text{, for all } A\in\cP(\cH).
\end{equation}
\begin{enumerate}
    \item If $0<p\leq1$ and $0<s\leq\frac{1}{p}$, then $\Upsilon_{p,s}(A)$ is concave;
    \item If $-1\leq p\leq0$ and $s>0$, then $\Upsilon_{p,s}(A)$ is convex;
    \item If $1\leq p\leq 2$ and $s\geq\frac{1}{p}$, then $\Upsilon_{p,s}(A)$ is convex.
\end{enumerate}
\end{theorem}









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Monotonicity result%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{proposition}\cite[Corollary 1.5]{CFLconjecture}\label{monotone}
When $\alpha>1$, $D_{\alpha,z}$ is monotone under quantum channels if and only if the map from (\ref{functional}) is monotone increasing under quantum channels. 
\end{proposition}

\begin{proof}
Suppose the map from (\ref{functional}) is monotone increasing under quantum channels. i.e., if $\Lambda$ is a quantum channel and $A\geq\Lambda(A)$ as operators, then monotonicity means $\Psi(A)\geq\Psi(\Lambda(A))$. Since the trace operation is a quantum channel this implies that 
\begin{equation}
\mathrm{Tr}(A^{\frac{q}{2}}IA^pIA^{\frac{q}{2}})^{\frac{1}{p+q}}\geq \mathrm{Tr}(\Lambda(A)^{\frac{q}{2}}I\Lambda(A)^pI\Lambda(A)^{\frac{q}{2}})^{\frac{1}{p+q}}.
\end{equation}
So by an argument made in \cite{summaryPaper}, it follows that 
$$\mathrm{Tr}(B^{\frac{q}{2}}A^pB^{\frac{q}{2}})^{\frac{1}{p+q}}\geq \mathrm{Tr}(\Lambda(B)^{\frac{q}{2}}\Lambda(A)^p\Lambda(B)^{\frac{q}{2}})^{\frac{1}{p+q}}.$$ Since $\alpha>1$ and using the fact that the log function is monotone increasing, we have that $D_{\alpha,z}(A||B)\geq D_{\alpha,z}(\Lambda(A)||\Lambda(B))$. The converse is trivial. 
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% some step by step stuff %%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{proposition}\label{algebraicsufficient}
If $\rho_{AB}\in\cD(\cH_{AB})$ is a product state and $\sigma_{AB}\in\cP(\cH_{AB})$ is any density operator such that they have the following structure, 
$$ \sigma_{AB}^{\frac{1-\alpha}{2z}}\left(\sigma_{AB}^{\frac{1-\alpha}{2z}}\rho_{AB}^{\frac{\alpha}{z}}\sigma_{AB}^{\frac{1-\alpha}{2z}}\right)^{z-1}\sigma_{AB}^{\frac{1-\alpha}{2z}}=\sigma_A^{\frac{1-\alpha}{2z}}\left(\sigma_A^{\frac{1-\alpha}{2z}}\rho_A^{\frac{\alpha}{z}}\sigma_A^{\frac{1-\alpha}{2z}}\right)^{z-1}\sigma_A^{\frac{1-\alpha}{2z}} \otimes\mathbbm{1}_B,$$ 
then the Data processing inequality under partial traces is saturated plus some constant. i.e., $$D_{\alpha,z}(\rho_{AB}||\sigma_{AB})=D_{\alpha,z}(\rho_A||\sigma_A) + k,$$
for some positive $k$. 
\end{proposition}

\begin{proof}
Since $\rho_{AB}$ is a product state on $\cH_{AB}$, it follows that $\rho_{AB}=\rho_A\otimes\rho_B$, where $\rho_A$ is a density operator on $\cH_A$ and $\rho_B$ is a density operator on $\cH_B$. Note that $\rho_B$ need not be a pure state. Hence we see \footnote{Note that we are using the fact that $\mathrm{Tr}_{AB}(X)=\mathrm{Tr}_A(\mathrm{Tr}_BX)$}
\begingroup
\allowdisplaybreaks
\begin{align}
    &\sigma_{AB}^{\frac{1-\alpha}{2z}}\left(\sigma_{AB}^{\frac{1-\alpha}{2z}}\rho_{AB}^{\frac{\alpha}{z}}\sigma_{AB}^{\frac{1-\alpha}{2z}}\right)^{z-1}\sigma_{AB}^{\frac{1-\alpha}{2z}} = \sigma_A^{\frac{1-\alpha}{2z}}\left(\sigma_A^{\frac{1-\alpha}{2z}}\rho_A^{\frac{\alpha}{z}}\sigma_A^{\frac{1-\alpha}{2z}}\right)^{z-1}\sigma_A^{\frac{1-\alpha}{2z}} \otimes\mathbbm{1}_B \\
    \implies & \rho_{AB}^\frac{\alpha}{z}\sigma_{AB}^{\frac{1-\alpha}{2z}}\left(\sigma_{AB}^{\frac{1-\alpha}{2z}}\rho_{AB}^{\frac{\alpha}{z}}\sigma_{AB}^{\frac{1-\alpha}{2z}}\right)^{z-1}\sigma_{AB}^{\frac{1-\alpha}{2z}} = \rho_{AB}^\frac{\alpha}{z}\left(\sigma_A^{\frac{1-\alpha}{2z}}\left(\sigma_A^{\frac{1-\alpha}{2z}}\rho_A^{\frac{\alpha}{z}}\sigma_A^{\frac{1-\alpha}{2z}}\right)^{z-1}\sigma_A^{\frac{1-\alpha}{2z}} \otimes\mathbbm{1}_B \right) \\
    \implies &
    \mathrm{Tr}\left(\rho_{AB}^\frac{\alpha}{z}\sigma_{AB}^{\frac{1-\alpha}{2z}}\left(\sigma_{AB}^{\frac{1-\alpha}{2z}}\rho_{AB}^{\frac{\alpha}{z}}\sigma_{AB}^{\frac{1-\alpha}{2z}}\right)^{z-1}\sigma_{AB}^{\frac{1-\alpha}{2z}}\right) = \mathrm{Tr}\left(\rho_{AB}^\frac{\alpha}{z}\left(\sigma_A^{\frac{1-\alpha}{2z}}\left(\sigma_A^{\frac{1-\alpha}{2z}}\rho_A^{\frac{\alpha}{z}}\sigma_A^{\frac{1-\alpha}{2z}}\right)^{z-1}\sigma_A^{\frac{1-\alpha}{2z}} \otimes\mathbbm{1}_B \right)\right)\\
    \implies & 
    \mathrm{Tr}\left[\left(\sigma_{AB}^{\frac{1-\alpha}{2z}}\rho_{AB}^{\frac{\alpha}{z}}\sigma_{AB}^{\frac{1-\alpha}{2z}}\right)^z\right] = \mathrm{Tr} \left((\rho_A\otimes\rho_B)^{\frac{\alpha}{z}}\sigma_A^{\frac{1-\alpha}{2z}}\left(\sigma_A^{\frac{1-\alpha}{2z}}\rho_A^{\frac{\alpha}{z}}\sigma_A^{\frac{1-\alpha}{2z}}\right)^{z-1}\sigma_A^{\frac{1-\alpha}{2z}}\right)\\
    \implies & 
    \mathrm{Tr}\left[\left(\sigma_{AB}^{\frac{1-\alpha}{2z}}\rho_{AB}^{\frac{\alpha}{z}}\sigma_{AB}^{\frac{1-\alpha}{2z}}\right)^z\right] = \mathrm{Tr} \left((\rho_A^{\frac{\alpha}{z}}\otimes\rho_B^{\frac{\alpha}{z}})\sigma_A^{\frac{1-\alpha}{2z}}\left(\sigma_A^{\frac{1-\alpha}{2z}}\rho_A^{\frac{\alpha}{z}}\sigma_A^{\frac{1-\alpha}{2z}}\right)^{z-1}\sigma_A^{\frac{1-\alpha}{2z}}\right)\\
    \implies &
     \mathrm{Tr}\left[\left(\sigma_{AB}^{\frac{1-\alpha}{2z}}\rho_{AB}^{\frac{\alpha}{z}}\sigma_{AB}^{\frac{1-\alpha}{2z}}\right)^z\right] = \mathrm{Tr}\left[ \left(\rho_A^{\frac{\alpha}{z}}\sigma_A^{\frac{1-\alpha}{2z}}\left(\sigma_A^{\frac{1-\alpha}{2z}}\rho_A^{\frac{\alpha}{z}}\sigma_A^{\frac{1-\alpha}{2z}}\right)^{z-1}\sigma_A^{\frac{1-\alpha}{2z}}\right)\otimes \rho_B^{\frac{\alpha}{z}}\right]\\
    \implies & 
     \mathrm{Tr}\left[\left(\sigma_{AB}^{\frac{1-\alpha}{2z}}\rho_{AB}^{\frac{\alpha}{z}}\sigma_{AB}^{\frac{1-\alpha}{2z}}\right)^z\right] = \mathrm{Tr}\left[ \left(\sigma_A^{\frac{1-\alpha}{2z}}\rho_A^{\frac{\alpha}{z}}\sigma_A^{\frac{1-\alpha}{2z}}\right)^{z}\otimes \rho_B^{\frac{\alpha}{z}}\right]\\
    \implies & 
     \mathrm{Tr}\left[\left(\sigma_{AB}^{\frac{1-\alpha}{2z}}\rho_{AB}^{\frac{\alpha}{z}}\sigma_{AB}^{\frac{1-\alpha}{2z}}\right)^z\right] = \mathrm{Tr}\left[ \left(\sigma_A^{\frac{1-\alpha}{2z}}\rho_A^{\frac{\alpha}{z}}\sigma_A^{\frac{1-\alpha}{2z}}\right)^{z}\right]\mathrm{Tr}\left( \rho_B^{\frac{\alpha}{z}}\right)\\
    \implies & 
         \frac{1}{\alpha-1}\log\left(\mathrm{Tr}\left[\left(\sigma_{AB}^{\frac{1-\alpha}{2z}}\rho_{AB}^{\frac{\alpha}{z}}\sigma_{AB}^{\frac{1-\alpha}{2z}}\right)^z\right]\right) = \frac{1}{\alpha-1}\log\left(\mathrm{Tr}\left[ \left(\sigma_A^{\frac{1-\alpha}{2z}}\rho_A^{\frac{\alpha}{z}}\sigma_A^{\frac{1-\alpha}{2z}}\right)^{z}\right]\mathrm{Tr}\left( \rho_B^{\frac{\alpha}{z}}\right)\right)\\
    \implies & 
         \frac{1}{\alpha-1}\log\left(\mathrm{Tr}\left[\left(\sigma_{AB}^{\frac{1-\alpha}{2z}}\rho_{AB}^{\frac{\alpha}{z}}\sigma_{AB}^{\frac{1-\alpha}{2z}}\right)^z\right]\right) = \frac{1}{\alpha-1}\log\left(\mathrm{Tr}\left[ \left(\sigma_A^{\frac{1-\alpha}{2z}}\rho_A^{\frac{\alpha}{z}}\sigma_A^{\frac{1-\alpha}{2z}}\right)^{z}\right]\right)+\frac{1}{\alpha-1}\log\left[\mathrm{Tr}\left(\rho_B^{\frac{\alpha}{z}}\right)\right]\\
    \implies &     
    D_{\alpha,z}(\rho_{AB}||\sigma_{AB}) = D_{\alpha,z}(\rho_A||\sigma_A) + k, 
\end{align}
\endgroup
where $k= \frac{1}{\alpha-1}\log\left[\mathrm{Tr}\left(\rho_B^{\frac{\alpha}{z}}\right)\right]$.  
\end{proof}




\begin{proposition}
If $\rho_{AB}\in\cD(\cH_{AB})$ is a separable state and $\sigma_{AB}\in\cP(\cH_{AB})$ is such that they have the following structure, 
$$ \sigma_{AB}^{\frac{1-\alpha}{2z}}\left(\sigma_{AB}^{\frac{1-\alpha}{2z}}\rho_{AB}^{\frac{\alpha}{z}}\sigma_{AB}^{\frac{1-\alpha}{2z}}\right)^{z-1}\sigma_{AB}^{\frac{1-\alpha}{2z}}=\sigma_A^{\frac{1-\alpha}{2z}}\left(\sigma_A^{\frac{1-\alpha}{2z}}\rho_A^{\frac{\alpha}{z}}\sigma_A^{\frac{1-\alpha}{2z}}\right)^{z-1}\sigma_A^{\frac{1-\alpha}{2z}},$$ 
then the Data processing inequality under partial traces is saturated. i.e., $$D_{\alpha,z}(\rho_{AB}||\sigma_{AB})=D_{\alpha,z}(\rho_A||\sigma_A).$$
\end{proposition}

\begin{proof}
Since $\rho_{AB}$ is a separable state on $\cH_{AB}$, we may write $\rho_{AB}$ as a convex combination of a tensor product of pure states. i.e., $\rho_{AB}=\sum\limits_{i\in I}\lambda_i\ket{\psi_i}_A\bra{\psi_i}\otimes\ket{\phi_i}_B\bra{\phi_i}$, where $\{\ket{\psi_i}\}$ and $\{\ket{\phi_i}\}$ are sets of pure states on $\cH_A$ and $\cH_B$ respectively, as well as $0\leq\lambda_i\leq1$, for all $i\in I$ so that $\sum\limits_{i\in I}\lambda_i=1$. Hence we have \footnote{Note that we are using the fact that $\mathrm{Tr}_{AB}(X)=\mathrm{Tr}_A(\mathrm{Tr}_BX)$}
\begingroup
\allowdisplaybreaks
\begin{align}
    &\sigma_{AB}^{\frac{1-\alpha}{2z}}\left(\sigma_{AB}^{\frac{1-\alpha}{2z}}\rho_{AB}^{\frac{\alpha}{z}}\sigma_{AB}^{\frac{1-\alpha}{2z}}\right)^{z-1}\sigma_{AB}^{\frac{1-\alpha}{2z}} = \sigma_A^{\frac{1-\alpha}{2z}}\left(\sigma_A^{\frac{1-\alpha}{2z}}\rho_A^{\frac{\alpha}{z}}\sigma_A^{\frac{1-\alpha}{2z}}\right)^{z-1}\sigma_A^{\frac{1-\alpha}{2z}} \otimes\mathbbm{1}_B \\
    \implies & 
    \rho_{AB}^\frac{\alpha}{z}\sigma_{AB}^{\frac{1-\alpha}{2z}}\left(\sigma_{AB}^{\frac{1-\alpha}{2z}}\rho_{AB}^{\frac{\alpha}{z}}\sigma_{AB}^{\frac{1-\alpha}{2z}}\right)^{z-1}\sigma_{AB}^{\frac{1-\alpha}{2z}} = \rho_{AB}^\frac{\alpha}{z}\left(\sigma_A^{\frac{1-\alpha}{2z}}\left(\sigma_A^{\frac{1-\alpha}{2z}}\rho_A^{\frac{\alpha}{z}}\sigma_A^{\frac{1-\alpha}{2z}}\right)^{z-1}\sigma_A^{\frac{1-\alpha}{2z}} \otimes\mathbbm{1}_B \right) \\
    \implies &
    \mathrm{Tr}\left(\rho_{AB}^\frac{\alpha}{z}\sigma_{AB}^{\frac{1-\alpha}{2z}}\left(\sigma_{AB}^{\frac{1-\alpha}{2z}}\rho_{AB}^{\frac{\alpha}{z}}\sigma_{AB}^{\frac{1-\alpha}{2z}}\right)^{z-1}\sigma_{AB}^{\frac{1-\alpha}{2z}}\right) = \mathrm{Tr}\left(\rho_{AB}^\frac{\alpha}{z}\left(\sigma_A^{\frac{1-\alpha}{2z}}\left(\sigma_A^{\frac{1-\alpha}{2z}}\rho_A^{\frac{\alpha}{z}}\sigma_A^{\frac{1-\alpha}{2z}}\right)^{z-1}\sigma_A^{\frac{1-\alpha}{2z}} \otimes\mathbbm{1}_B \right)\right)\\
    \implies & 
    \mathrm{Tr}\left[\left(\sigma_{AB}^{\frac{1-\alpha}{2z}}\rho_{AB}^{\frac{\alpha}{z}}\sigma_{AB}^{\frac{1-\alpha}{2z}}\right)^z\right] = \mathrm{Tr} \left(\left(\sum_{i\in I}\lambda_i\ket{\psi_i}_A\bra{\psi_i}\otimes\ket{\phi_i}_B\bra{\phi_i}\right)^{\frac{\alpha}{z}}\sigma_A^{\frac{1-\alpha}{2z}}\left(\sigma_A^{\frac{1-\alpha}{2z}}\rho_A^{\frac{\alpha}{z}}\sigma_A^{\frac{1-\alpha}{2z}}\right)^{z-1}\sigma_A^{\frac{1-\alpha}{2z}}\right)\\
    \implies & 
    \mathrm{Tr}\left[\left(\sigma_{AB}^{\frac{1-\alpha}{2z}}\rho_{AB}^{\frac{\alpha}{z}}\sigma_{AB}^{\frac{1-\alpha}{2z}}\right)^z\right] = \mathrm{Tr} \left(\left(\sum_{i\in I}\lambda_i^{\frac{\alpha}{z}}\ket{\psi_i}_A\bra{\psi_i}\otimes\ket{\phi_i}_B\bra{\phi_i}\right)\sigma_A^{\frac{1-\alpha}{2z}}\left(\sigma_A^{\frac{1-\alpha}{2z}}\rho_A^{\frac{\alpha}{z}}\sigma_A^{\frac{1-\alpha}{2z}}\right)^{z-1}\sigma_A^{\frac{1-\alpha}{2z}}\right)\\
    \implies &
     \mathrm{Tr}\left[\left(\sigma_{AB}^{\frac{1-\alpha}{2z}}\rho_{AB}^{\frac{\alpha}{z}}\sigma_{AB}^{\frac{1-\alpha}{2z}}\right)^z\right] = \mathrm{Tr}\left[ \left(\left(\sum_{i\in I}\lambda_i^{\frac{\alpha}{z}}\ket{\psi_i}_A\bra{\psi_i}\right)\sigma_A^{\frac{1-\alpha}{2z}}\left(\sigma_A^{\frac{1-\alpha}{2z}}\rho_A^{\frac{\alpha}{z}}\sigma_A^{\frac{1-\alpha}{2z}}\right)^{z-1}\sigma_A^{\frac{1-\alpha}{2z}}\right)\otimes\ket{\phi_i}_B\bra{\phi_i}\right]\\
    \implies & 
         \mathrm{Tr}\left[\left(\sigma_{AB}^{\frac{1-\alpha}{2z}}\rho_{AB}^{\frac{\alpha}{z}}\sigma_{AB}^{\frac{1-\alpha}{2z}}\right)^z\right] = \mathrm{Tr}\left[ \left(\rho_A^{\frac{\alpha}{z}}\sigma_A^{\frac{1-\alpha}{2z}}\left(\sigma_A^{\frac{1-\alpha}{2z}}\rho_A^{\frac{\alpha}{z}}\sigma_A^{\frac{1-\alpha}{2z}}\right)^{z-1}\sigma_A^{\frac{1-\alpha}{2z}}\right)\right]\\
    \implies & 
     \mathrm{Tr}\left[\left(\sigma_{AB}^{\frac{1-\alpha}{2z}}\rho_{AB}^{\frac{\alpha}{z}}\sigma_{AB}^{\frac{1-\alpha}{2z}}\right)^z\right] = \mathrm{Tr}\left[ \left(\sigma_A^{\frac{1-\alpha}{2z}}\rho_A^{\frac{\alpha}{z}}\sigma_A^{\frac{1-\alpha}{2z}}\right)^{z}\right]\\
    \implies & 
     \mathrm{Tr}\left[\left(\sigma_{AB}^{\frac{1-\alpha}{2z}}\rho_{AB}^{\frac{\alpha}{z}}\sigma_{AB}^{\frac{1-\alpha}{2z}}\right)^z\right] = \mathrm{Tr}\left[ \left(\sigma_A^{\frac{1-\alpha}{2z}}\rho_A^{\frac{\alpha}{z}}\sigma_A^{\frac{1-\alpha}{2z}}\right)^{z}\right]\\
    \implies & 
         \frac{1}{\alpha-1}\log\left(\mathrm{Tr}\left[\left(\sigma_{AB}^{\frac{1-\alpha}{2z}}\rho_{AB}^{\frac{\alpha}{z}}\sigma_{AB}^{\frac{1-\alpha}{2z}}\right)^z\right]\right) = \frac{1}{\alpha-1}\log\left(\mathrm{Tr}\left[ \left(\sigma_A^{\frac{1-\alpha}{2z}}\rho_A^{\frac{\alpha}{z}}\sigma_A^{\frac{1-\alpha}{2z}}\right)^{z}\right]\right)\\
    \implies & 
    D_{\alpha,z}(\rho_{AB}||\sigma_{AB}) = D_{\alpha,z}(\rho_A||\sigma_A), 
\end{align}
\endgroup
as desired.
\end{proof}










%%%% sup of convex is convex  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{proposition}\label{maxconvex}
If $f(A,B,H)$ is jointly convex in $A$ and $B$, then so is $$\sup_{H>0}\{f(A,B,H)\}.$$
\end{proposition}

\begin{proof}
Given that $f$ is jointly convex in $A$ and $B$, we have that for given $0\leq\lambda_i\leq1$ such that $\sum\limits_i\lambda_i=1$, the following is true
$$f\left(\sum_i\lambda_iA_i, \sum_i\lambda_iB_i, H\right) \leq \sum_i\lambda_if(A_i,B_i,H).$$ Thus for every positive $H$, we have that  $\sum_i\lambda_if(A_i,B_i,H)$ is an upper bound for $f\left(\sum_i\lambda_iA_i, \sum_i\lambda_iB_i, H\right)$, and hence  $$\sup_{H>0}\left\{f\left(\sum_i\lambda_iA_i, \sum_i\lambda_iB_i, H\right)\right\} \leq \sup\limits_{H>0}\left\{ \sum_i\lambda_if(A_i,B_i,H)\right\}.$$ Since for all $i$, we have that $\lambda_i\geq0$, it follows that
$$\sup_{H>0}\left\{f\left(\sum_i\lambda_iA_i, \sum_i\lambda_iB_i, H\right)\right\} \leq \sum_i \lambda_i \sup_{H>0}\{f(A_i,B_i,H)\},$$
as desired. 
\end{proof}




%%%%%%%%%%%%%%%%%%
%Z^* inverse
%%%%%%%%%%%%%%%%%%

\begin{lemma}\label{z*inverse}
For any invertible operator $Z$, we have that $(Z^*)^{-1}=(Z^{-1})^*$.
\end{lemma}

\begin{proof}
 For any $y$, since 
\begin{align}
    \langle Z^*(Z^{-1})^*y,y\rangle 
    & = \langle (Z^{-1})^*y,Zy\rangle \\
    & = \langle y,Z^{-1}Zy\rangle \\
    & = \langle y,y\rangle,
\end{align}
it follows that $Z^*(Z^{-1})^* = \mathbbm{1}$, and similarly, $(Z^{-1})^*Z^* = \mathbbm{1}$ so then $(Z^*)^{-1} = (Z^{-1})^*$.
\end{proof}


==> prelims.tex <==

%%%%%%%%%%% f function %%%%%%%%%%%%


%%%%%%%%%%% f function %%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%% convexity of f %%%%%%%%%%%%


To prove joint convexity of $f_{\alpha, z}(H,\rho, \sigma)$ from equation (\ref{f1}), the next few results are required. Recall the equation from (\ref{functional})
\begin{equation}\label{functional1}
(A,B)\mapsto\mathrm{Tr}(B^{\frac{q}{2}}K^*A^pKB^{\frac{q}{2}})^s.
\end{equation}

\begin{theorem}\cite[Theorem 1.1]{CFLconjecture}\label{Reduced1}
Fix any invertible matrix $\cK$. Suppose that $p\geq q$ and $s>0$. 
\begin{enumerate}
    \item If $0\leq q\leq p\leq 1$ and $0<s\leq\frac{1}{p+q}$, then the map from (\ref{functional1}) is jointly concave.
    \item If $-1\leq q\leq p\leq 0$ and $s>0$, then the map from (\ref{functional1}) is jointly convex. 
    \item If $-1\leq q \leq 0$, $1\leq p\leq2$, $(p,q)\neq (1,-1)$ and $s\geq\frac{1}{p+q}$, then the map from (\ref{functional1}) is jointly convex.
\end{enumerate}
\end{theorem}

\begin{theorem}\cite[Theorem 3.3]{CFLconjecture}\label{zhangresult}
For $r_i>0$, $i\in\{0,1,2\}$ such that $\frac{1}{r_0}=\frac{1}{r_1}+\frac{1}{r_2}$, we have that for any invertible $X,Y\in\cB(\cH)$ that
\begin{equation}
    \mathrm{Tr}|XY|^{r_1} = \max\left\{ \frac{r_1}{r_0} \mathrm{Tr}|XZ|^{r_0}-\frac{r_1}{r_2}\mathrm{Tr}|Y^{-1}Z|^{r_2} : Z\in\cB(\cH) \text{ and invertible} \right\}.
\end{equation}

\end{theorem}

\begin{proposition}\cite[Proposition 5]{summaryPaper}\label{fixedB}
For a fixed operator $B$, the map on positive operators 
$$A\mapsto \mathrm{Tr}\left[(B^*A^pB)^{\frac{1}{p}}\right] $$ \begin{enumerate}
    \item is concave for $0\leq p\leq 1$, with $p\neq0$.
    \item is convex for $1\leq p\leq 2$, with $p\neq0$.
\end{enumerate}
\end{proposition}

\begin{proposition}\label{sum}
If $f:\cD(\cH)\times\cD(\cH)\times\cP(\cH)\mapsto[0,\infty)$ is defined as 
$$f(A,B,H) := g(A,H) + h(B,H), $$
where $g$ and $h$ are continuous, the functional $g$ is convex in $A$ and the functional $h$ is convex in $B$, then $f$ is jointly convex in $(A,B)$. 
\end{proposition}

\begin{proof}
For all $i$ such that $0\leq\lambda_i\leq1$, with $\sum_i\lambda_i=1$, by convexity of $g$ and $h$, 
$$g\left(\sum_i\lambda_iA_i, H\right) \leq \sum_i\lambda_ig(A_i, H) $$ and 
$$h\left(\sum_i\lambda_iB_i, H\right) \leq \sum_i\lambda_ih(B_i, H). $$
Thus
\begin{align}
    f\left(\sum_i\lambda_iA_i,\sum_i\lambda_iB_i,H \right) & = g\left(\sum_i\lambda_iA_i, H\right) + h\left(\sum_i\lambda_iB_i, H\right) \\
    & \leq \sum_i\lambda_ig(A_i, H) + \sum_i\lambda_ih(B_i, H) \\
    & = \sum_i\lambda_i\left(g(A_i, H) + h(B_i, H)\right) \\
    & = f(A_i, B_i, H),
\end{align}
as desired. 
\end{proof}

\begin{proposition}\label{maxconvex}
If $f(A,B,H)$ is jointly convex in $A$ and $B$, then so is $$\sup_{H>0}\{f(A,B,H)\}.$$
\end{proposition}






%%%%%%%%%%% convexity of f %%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Certain Trace Functional and its Convexity}


Here are the technical results that helped us prove the main result.   Recall that $$\Psi_{\alpha,z}(\rho||\sigma):=\mathrm{Tr}\left[\left(\sigma^{\frac{1-\alpha}{2z}}\rho^{\frac{\alpha}{z}}\sigma^{\frac{1-\alpha}{2z}}\right)^z\right]. $$

\begin{lemma}\label{function2}
Let $\rho$ and $\sigma\in\cD(\cH)$, and assume that $\alpha>1$ and $z>1$. For any positive operator $H$, define
\begin{equation}\label{f1}
     f_{\alpha,z}(H,\rho,\sigma) :=      z\mathrm{Tr}(\sigma^{\frac{z-\alpha}{2z}}\rho^{\frac{\alpha}{z}}\sigma^{\frac{z-\alpha}{2z}}H) - (z-1)\mathrm{Tr}\left[(\sigma^{\frac{z-1}{2z}}H\sigma^{\frac{z-1}{2z}})^{\frac{z}{z-1}}\right].
\end{equation}
Then
\begin{equation}
    \Psi_{\alpha,z}(\rho||\sigma)=\sup_{H>0} f_{\alpha,z,H}(\rho,\sigma),
\end{equation}
where the supremum is achieved whenever $H = \sigma^{\frac{1-z}{2z}}(\sigma^{\frac{1-\alpha}{2z}}\rho^{\frac{\alpha}{z}}\sigma^{\frac{1-\alpha}{2z}})^{z-1}\sigma^{\frac{1-z}{2z}}$. 

\end{lemma}
\begin{proof}

For $X$ and $Y$ $\in\cP(\cH)$, and for a choice of  $1\leq p,q\leq\infty$, such that $1=\frac{1}{p}+\frac{1}{q}$, one has
\begin{align}
    \mathrm{Tr}(XY) =& \mathrm{Tr}(X^*Y) \label{xpos1}\\
    \leq& |\mathrm{Tr}(X^*Y)| \\
    \leq& \left(\mathrm{Tr}|X|^p\right)^{\frac{1}{P}}\left(\mathrm{Tr}|Y|^q\right)^{\frac{1}{q}} \label{baug1}\\
    =& \left(\mathrm{Tr}X^p\right)^{\frac{1}{P}}\left(\mathrm{Tr}Y^q\right)^{\frac{1}{q}} \label{sa} \label{xypos1}\\
    \leq& \frac{1}{p}\mathrm{Tr}X^p + \frac{1}{q} \mathrm{Tr}Y^q, \label{young1}
\end{align}
where (\ref{xpos1}) is from the assumption that $X$ is positive, (\ref{baug1}) is from Theorem 2 in \cite{baumgartner}, (\ref{sa}) is because $X$ and $Y$ are self adjoint, and (\ref{young1}) is from Young's inequality stated as Theorem \ref{Young}. 
Thus, 
\begin{equation}\label{inequality1}
    p\mathrm{Tr}(XY) - \frac{p}{q}\mathrm{Tr}(Y)^{q} \leq \mathrm{Tr}X^{p},
\end{equation}
 with equality if and only if 
$ X^{p}=Y^{q}.$
Take  positive operators 
$$ X=(\sigma^{\frac{1-\alpha}{2z}}\rho^{\frac{\alpha}{z}}\sigma^{\frac{1-\alpha}{2z}}) \text{ and } Y=(\sigma^{\frac{z-1}{2z}}H\sigma^{\frac{z-1}{2z}}), $$
where $H$ is some positive operator in $\cB(\cH)$. Then (\ref{inequality1}) becomes
\begin{equation}\label{newIneq1}
    p\mathrm{Tr}(\sigma^{\frac{1-\alpha}{2z}}\rho^{\frac{\alpha}{z}}\sigma^{\frac{1-\alpha}{2z}}\sigma^{\frac{z-1}{2z}}H\sigma^{\frac{z-1}{2z}}) - \frac{p}{q}\mathrm{Tr}\left[(\sigma^{\frac{z-1}{2z}}H\sigma^{\frac{z-1}{2z}})^{q}\right] \leq \mathrm{Tr}\left[(\sigma^{\frac{1-\alpha}{2z}}\rho^{\frac{\alpha}{z}}\sigma^{\frac{1-\alpha}{2z}})^{p}\right].
\end{equation}
Equality happens 
\begin{align}
    \text{if and only if } & X^{p}=Y^{q} \\
    \text{if and only if } & \left(\sigma^{\frac{1-\alpha}{2z}}\rho^{\frac{\alpha}{z}}\sigma^{\frac{1-\alpha}{2z}}\right)^{p}=\left(\sigma^{\frac{z-1}{2z}}H\sigma^{\frac{z-1}{2z}}\right)^{q} \\
    \text{if and only if } & \sigma^{\frac{1-z}{2z}}\left(\sigma^{\frac{1-\alpha}{2z}}\rho^{\frac{\alpha}{z}}\sigma^{\frac{1-\alpha}{2z}}\right)^{\frac{p}{q}}\sigma^{\frac{1-z}{2z}}=H.
\end{align} 
By construction, $H$ is unique, hence the left hand side of (\ref{inequality1}) becomes 
\begin{align}
     &\hspace*{-1cm} p\mathrm{Tr}\left(\sigma^{\frac{1-\alpha}{2z}}\rho^{\frac{\alpha}{z}}\sigma^{\frac{1-\alpha}{2z}}\sigma^{\frac{z-1}{2z}}\sigma^{\frac{1-z}{2z}}\left(\sigma^{\frac{1-\alpha}{2z}}\rho^{\frac{\alpha}{z}}\sigma^{\frac{1-\alpha}{2z}}\right)^{\frac{p}{q}}\sigma^{\frac{1-z}{2z}}\sigma^{\frac{z-1}{2z}}\right) - \frac{p}{q}\mathrm{Tr}\left[\left(\sigma^{\frac{z-1}{2z}}\sigma^{\frac{1-z}{2z}}\left(\sigma^{\frac{1-\alpha}{2z}}\rho^{\frac{\alpha}{z}}\sigma^{\frac{1-\alpha}{2z}}\right)^{\frac{p}{q}}\sigma^{\frac{1-z}{2z}}\sigma^{\frac{z-1}{2z}}\right)^{q}\right] \\
     = & p\mathrm{Tr}\left(\sigma^{\frac{1-\alpha}{2z}}\rho^{\frac{\alpha}{z}}\sigma^{\frac{1-\alpha}{2z}}\left(\sigma^{\frac{1-\alpha}{2z}}\rho^{\frac{\alpha}{z}}\sigma^{\frac{1-\alpha}{2z}}\right)^{\frac{p}{q}}\right) - \frac{p}{q}\mathrm{Tr}\left[\left(\left(\sigma^{\frac{1-\alpha}{2z}}\rho^{\frac{\alpha}{z}}\sigma^{\frac{1-\alpha}{2z}}\right)^{\frac{p}{q}}\right)^{q}\right] \\
     = & p\mathrm{Tr}\left(\left(\sigma^{\frac{1-\alpha}{2z}}\rho^{\frac{\alpha}{z}}\sigma^{\frac{1-\alpha}{2z}}\right)^{\frac{p}{q}+1}\right) - \frac{p}{q}\mathrm{Tr}\left[\left(\sigma^{\frac{1-\alpha}{2z}}\rho^{\frac{\alpha}{z}}\sigma^{\frac{1-\alpha}{2z}}\right)^p\right] \\
     = & \left(p-\frac{p}{q}\right)\mathrm{Tr}\left[\left(\sigma^{\frac{1-\alpha}{2z}}\rho^{\frac{\alpha}{z}}\sigma^{\frac{1-\alpha}{2z}}\right)^p\right]
     \\
     = & \mathrm{Tr}\left[\left(\sigma^{\frac{1-\alpha}{2z}}\rho^{\frac{\alpha}{z}}\sigma^{\frac{1-\alpha}{2z}}\right)^p\right].
\end{align}
where $1=\frac{1}{p}+\frac{1}{q}$ implies that $p+q=pq$ which implies $\frac{p}{q}+1 = p$ and $p-\frac{p}{q}=1$. For a choice of $p=z$ and $q=\frac{z}{z-1}$, where $z>1$, define the left hand side of (\ref{newIneq1}) as 
\begin{equation}\label{function1}
    f_{\alpha,z}(H,\rho,\sigma) :=      z\mathrm{Tr}(\sigma^{\frac{z-\alpha}{2z}}\rho^{\frac{\alpha}{z}}\sigma^{\frac{z-\alpha}{2z}}H) - (z-1)\mathrm{Tr}\left[(\sigma^{\frac{z-1}{2z}}H\sigma^{\frac{z-1}{2z}})^{\frac{z}{z-1}}\right].
\end{equation} Then the desired result is obtained.
\end{proof}



\begin{proposition}\label{jconvexity}
Whenever $1<z\leq \alpha\leq 2z$ and for a fixed $H>0$, one has that $f_{\alpha,z}(H,\rho,\sigma)$ from equation (\ref{f1}) is jointly convex in $\rho$ and $\sigma$. 
\end{proposition}

\begin{proof}
Fix $H>0$. Let $p = \frac{\alpha}{z}$, $q = \frac{z-\alpha}{z}$, $X=\rho^{\frac{p}{2}}$, and $Y = \sigma^{\frac{q}{2}}H^{\frac{1}{2}}$. Then $X$ is invertible because $\rho$ is, and similarly, $Y$ is invertible because $H$ and $\sigma$ are. Note that \begin{align}
    \mathrm{Tr}\left(\sigma^{\frac{z-\alpha}{2z}}\rho^{\frac{\alpha}{z}}\sigma^{\frac{z-\alpha}{2z}}H\right) & = \mathrm{Tr}\left(H^{\frac{1}{2}}\sigma^{\frac{z-\alpha}{2z}}\rho^{\frac{\alpha}{z}}\sigma^{\frac{z-\alpha}{2z}}H^{\frac{1}{2}}\right) \\
    & = \mathrm{Tr}\left(H^{\frac{1}{2}}\sigma^{\frac{z-\alpha}{2z}}\rho^{\frac{\alpha}{2z}}\rho^{\frac{\alpha}{2z}}\sigma^{\frac{z-\alpha}{2z}}H^{\frac{1}{2}}\right) \\
    & = \mathrm{Tr}\left(H^{\frac{1}{2}}\sigma^{\frac{q}{2}}\rho^{\frac{p}{2}}\rho^{\frac{p}{2}}\sigma^{\frac{q}{2}}H^{\frac{1}{2}}\right)\\
    & = \mathrm{Tr}\left(Y^*X^*XY\right)\\
    & = \mathrm{Tr}|XY|^2.
\end{align}
Since $1<z\leq\alpha\leq 2z$, it follows that $1\leq p = \frac{\alpha}{z}\leq 2$ and $0\leq -q = -\frac{z-\alpha}{z}\leq 1$. Both $p$ and $-q$ are both positive numbers, so set $(r_0,r_1,r_2) = (\frac{2}{p},2,-\frac{2}{q})$. 
Then by Theorem \ref{zhangresult},
\begin{equation}\label{partialsup}
\mathrm{Tr}\left(\sigma^{\frac{z-\alpha}{2z}}\rho^{\frac{\alpha}{z}}\sigma^{\frac{z-\alpha}{2z}}H\right) = \max\left\{ p\mathrm{Tr}|\rho^{\frac{p}{2}}Z|^{\frac{2}{p}}+q\mathrm{Tr}|H^{-\frac{1}{2}}\sigma^{-\frac{q}{2}}Z|^{-\frac{2}{q}} \right\},
\end{equation}
where $Z$ is invertible. Since $1\leq p\leq 2$, it follows from Proposition \ref{fixedB} part 2 that 
$$\rho\mapsto \mathrm{Tr}|\rho^{\frac{p}{2}}Z|^{\frac{2}{p}} = \mathrm{Tr}\left[\left(Z^*\rho^p Z\right)^{\frac{1}{p}}\right] $$ is convex in $\rho$. 
For the second term in (\ref{partialsup}), choose $\Phi_Z(X):= Z^*XZ$, which is linear, positive, and self adjoint. Let $\sigma = X$, $-q=p$, and $A=Z^{-1}H^{-1}(Z^{-1})^*$. Then $A$ is positive. Moreover, for any $y$, since 
\begin{align}
    \langle Z^*(Z^{-1})^*y,y\rangle 
    & = \langle (Z^{-1})^*y,Zy\rangle \\
    & = \langle y,Z^{-1}Zy\rangle \\
    & = \langle y,y\rangle,
\end{align}
it follows that $Z^*(Z^{-1})^* = \mathbbm{1}$, and similarly, $(Z^{-1})^*Z^* = \mathbbm{1}$ so then $(Z^*)^{-1} = (Z^{-1})^*$. Thus rewrite $A= Z^{-1}H^{-1}(Z^*)^{-1}$. Then by Proposition \ref{newPick},
\begin{align}
    \mathrm{Tr}|H^{-\frac{1}{2}}\sigma^{-\frac{q}{2}}Z|^{-\frac{2}{q}} & = \mathrm{Tr}\left(\left[(H^{-\frac{1}{2}}\sigma^{-\frac{q}{2}}Z)^*(H^{-\frac{1}{2}}\sigma^{-\frac{q}{2}}Z)\right]^{-\frac{1}{q}}\right) \\
    & = \mathrm{Tr}\left(\left[Z^*\sigma^{-\frac{q}{2}}H^{-1}\sigma^{-\frac{q}{2}}Z\right]^{-\frac{1}{q}}\right) \\
    & = \mathrm{Tr}\left(\left[Z^*\sigma^{-\frac{q}{2}}ZZ^{-1}H^{-1}(Z^*)^{-1}Z^*\sigma^{-\frac{q}{2}}Z\right]^{-\frac{1}{q}}\right) \\
    & = \mathrm{Tr}\left[\left\{\Phi_Z\left(X^{\frac{p}{2}}\right)A \,\Phi_Z\left(X^{\frac{p}{2}}\right)\right\}^{\frac{1}{p}}\right]
\end{align} is concave in $\sigma$. Since $q<0$, it follow that 
$$\sigma\mapsto q\mathrm{Tr}|H^{-\frac{1}{2}}\sigma^{-\frac{q}{2}}Z|^{-\frac{2}{q}} $$ is convex in $\sigma$. By Propositions \ref{sum} and \ref{maxconvex}, one concludes that $\mathrm{Tr}\left(\sigma^{\frac{z-\alpha}{2z}}\rho^{\frac{\alpha}{z}}\sigma^{\frac{z-\alpha}{2z}}H\right)$ is the maximum of a sum of two convex functionals and thus is itself convex in $\rho$ and $\sigma$. 
$ $ 

%%%%%%%%%%%%%%%%%%%%%%%%%

On the other hand, since $\sigma^{\frac{z-1}{2z}}H\sigma^{\frac{z-1}{2z}}$ and $H^{\frac{1}{2}}\sigma^{\frac{z-1}{z}}H^{\frac{1}{2}}$ have the same nonzero eigenvalues,  
$$\mathrm{Tr}\left(\left[\sigma^{\frac{z-1}{2z}}H\sigma^{\frac{z-1}{2z}}\right]^{\frac{z}{z-1}}\right)=\mathrm{Tr}\left(\left[H^{\frac{1}{2}}\sigma^{\frac{z-1}{z}}H^{\frac{1}{2}}\right]^{\frac{z}{z-1}}\right).$$
So choosing $B=H^{\frac{1}{2}}$, $A=\sigma$, and $p=\frac{z-1}{z}$, by Proposition \ref{fixedB} part 1, $\mathrm{Tr}\left(\left[\sigma^{\frac{z-1}{2z}}H\sigma^{\frac{z-1}{2z}}\right]^{\frac{z}{z-1}}\right)$ is concave in $\sigma$ whenever $0\leq\frac{z-1}{z}\leq 1$. Hence $$-(z-1)\mathrm{Tr}\left(\left[\sigma^{\frac{z-1}{2z}}H\sigma^{\frac{z-1}{2z}}\right]^{\frac{z}{z-1}}\right)$$ is convex in $\sigma$.By Proposition \ref{sum},
$$ f_{\alpha,z}(H,\rho,\sigma)=      z\mathrm{Tr}\left(\sigma^{\frac{z-\alpha}{2z}}\rho^{\frac{\alpha}{z}}\sigma^{\frac{z-\alpha}{2z}}H\right) - (z-1)\mathrm{Tr}\left(\left[\sigma^{\frac{z-1}{2z}}H\sigma^{\frac{z-1}{2z}}\right]^{\frac{z}{z-1}}\right) $$ is a sum of two convex functionals in $\rho$ and $\sigma$ as desired. 
\end{proof}

